Personalized Text-to-Image Generation with Auto-Regressive Models

Personalized image synthesis has emerged as a pivotal application in text-to-image generation, enabling the creation of images featuring specific subjects in diverse contexts. While diffusion models have dominated this domain, auto-regressive models, with their unified architecture for text and image modeling, remain underexplored for personalized image generation. This paper investigates the potential of optimizing auto-regressive models for personalized image synthesis, leveraging their inherent multimodal capabilities to perform this task. We propose a two-stage training strategy that combines optimization of text embeddings and fine-tuning of transformer layers. Our experiments on the auto-regressive model demonstrate that this method achieves comparable subject fidelity and prompt following to the leading diffusion-based personalization methods. The results highlight the effectiveness of auto-regressive models in personalized image generation, offering a new direction for future research in this area.

==> tables/lumina.tex <==
\begin{table*}[tbp]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}
{l | r | ccc | ccc | ccc}
\toprule 
\multirow{2}{*}{Rank} & \# Tranable & \multicolumn{3}{c |}{$N = 1$} & \multicolumn{3}{c |}{$N = 2$} & \multicolumn{3}{c }{$N = 4$} \\

& Parameters& DINO $\uparrow$ & CLIP-I $\uparrow$  & CLIP-T $\uparrow$  & DINO $\uparrow$ & CLIP-I $\uparrow$ & CLIP-T $\uparrow$ & DINO $\uparrow$ & CLIP-I $\uparrow$ & CLIP-T $\uparrow$  \\

\cmidrule(lr){1-2} \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
$r=16$ & 12M & 0.657 & 0.781 & 0.316 & 0.640 & 0.773 & 0.316 & 0.630 & 0.769& 0.319 \\

$r=64$ & 50M & 0.657 & 0.778 & 0.312& 0.656 & 0.777 & 0.315 & 0.638 & 0.769 & 0.317  \\

$r=256$ & 201M & \textbf{0.668} & 0.785 & 0.312 & 0.654 & 0.775 & 0.315 & 0.111 & 0.111 & 0.111  \\

\bottomrule
\end{tabular}%
}
\caption{\textbf{Quantitative results comparison of subject fidelity (DINO, CLIP-I) and prompt following (CLIP-T) under different training configuration of Lumina-mGPT.} For all the three metrics, scores are between 0 and 1, a higher score indicates better performance. \textbf{Bold} signifies the highest score under each configuration. 
}
\label{tab:lumina}
\end{table*}
